Characterizing and Understanding Software Developer Networks in Security Development

To build secure software, developers often work together during software development and maintenance to find, fix, and prevent security vulnerabilities. Examining the nature of developer interactions during their security activities regarding security introducing and fixing activities can provide insights for improving current practices. In this work, we conduct a large-scale empirical study to characterize and understand developers' interactions during their security activities regarding security introducing and fixing, which involves more than 16K security fixing commits and over 28K security introducing commits from nine large-scale open-source software projects. For our analysis, we first examine whether a project is a hero-centric project when assessing developers' contribution in their security activities. Then we study the interaction patterns between developers, explore how the distribution of the patterns changes over time, and study the impact of developers' interactions on the quality of projects. In addition, we also characterize the nature of developer interaction in security activities in comparison to developer interaction in non-security activities (i.e., introducing and fixing non-security bugs). Among our findings we identify that: most of the experimental projects are non hero-centric projects when evaluating developers' contribution by using their security activities; there exist common dominating interaction patterns across our experimental projects; the distribution of interaction patterns has correlation with the quality of software projects. We believe the findings from this study can help developers understand how vulnerabilitiesoriginate and fix under the interactions of software developers.

==> figure/80_x_percent_devs.tex <==
\begin{figure*}[!htb]
\centering
\includegraphics[width=0.9\textwidth]{figure/80_x_percent_devs.png}
\caption{The percentages of developers involved when contributing 80\% of a specific type of commits.}
\label{fig:80_20}
\end{figure*}

==> figure/RQ1.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=0.5\textwidth]{figure/rq1.png}
\caption{The distribution of developer interaction patterns during security activities.}
\label{fig:secDist}
\vspace{-0.15in}
\end{figure}

==> figure/RQ2.tex <==
\begin{figure}[!tb]
\centering
\includegraphics[width=0.5\textwidth]{figure/rq2.png}
\caption{The distribution of developer interaction during non-security activities.}
\label{fig:disNonSec}
\end{figure}

==> figure/distribution/dist_non_security.tex <==
\begin{figure}[th!]
\centering
\scriptsize
\input{figure/distribution/non_security.tex}
\caption{\small The distribution of developer interaction during non-security activities.}
\label{fig:disNonSec}
\vspace{-0.1in}
\end{figure}

==> figure/distribution/dist_security.tex <==
\begin{figure}[th!]
\centering
\scriptsize
\input{figure/distribution/security.tex}
\caption{\small The distribution of developer interaction patterns during security activities.}
\label{fig:secDist}
\end{figure}

==> figure/distribution/non_security.tex <==
\begin{tikzpicture}
\begin{axis}[
ybar stacked,
height=4.5cm,
width = 9.7cm,
enlargelimits=0.1,
legend style={at={(0.5,-0.12)},
anchor=north,legend columns=-1},
%color ={black!3, black!10, black!20, black!30, black!40, black!50, black!55, black!60, black!65, black!70}
%ylabel={\#participants},
symbolic x coords={FFmpeg, freebsd, gcc, node, panda, php, qemu, linux, android},
xtick=data,
x tick label style={font=\scriptsize},
]
\addplot+[ybar,black!10,  fill=black!10]coordinates{(FFmpeg, 0.303889188) (freebsd, 0.40424316) (gcc,0.372938969) (node,0.590264978) (panda,0.394006504) (php, 0.42747393) (qemu, 0.354258403) (linux, 0.321312975) (android,0.29079486)};
\addplot+[ybar,black!30,  fill=black!30]coordinates{(FFmpeg, 0.14758021) (freebsd, 0.114086952) (gcc,0.261061999) (node, 0.263193116) (panda, 0.041657322) (php, 0.161634798) (qemu, 0.196991303) (linux, 0.154650236) (android, 0.20822418)};
\addplot+[ybar,black!50,  fill=black!50]coordinates{(FFmpeg, 0.315432057) (freebsd, 0.302503281) (gcc,0.223978189) (node, 0.097080198) (panda, 0.356470061) (php, 0.253470403) (qemu, 0.28443156) (linux, 0.330268985) (android, 0.278943966)};


\addplot+[ybar,black!65,  fill=black!65]coordinates{(FFmpeg, 0.031561742) (freebsd, 0.025505524) (gcc,0.023581621) (node, 0.015285817) (panda, 0.039498767) (php, 0.036530557) (qemu, 0.043923842) (linux, 0.035406805) (android, 0.057088422)};

\addplot+[ybar,black!75,  fill=black!75]coordinates{(FFmpeg, 0.197610542) (freebsd, 0.153301254) (gcc, 0.116633423) (node, 0.033753243) (panda, 0.16646109) (php, 0.119908784) (qemu, 0.11923529) (linux, 0.158212679) (android, 0.163530999)};

\addplot+[ybar,black!100,  fill=black!100]coordinates{(FFmpeg, 0.00392626) (freebsd, 0.000359829) (gcc, 0.0018058) (node, 0.000422649) (panda, 0.001906257) (php, 0.000981528) (qemu, 0.001159602) (linux,0.00014832) (android, 0.001417571)};

\legend{P1, P2, P3, P4, P5, P6}
\end{axis}
\end{tikzpicture}

==> figure/distribution/security.tex <==
\begin{tikzpicture}
\begin{axis}[
ybar stacked,
height=4.5cm,
width = 9.7cm,
enlargelimits=0.1,
legend style={at={(0.5,-0.12)},
anchor=north,legend columns=-1},
%color ={black!3, black!10, black!20, black!30, black!40, black!50, black!55, black!60, black!65, black!70}
%ylabel={\#participants},
symbolic x coords={FFmpeg, freebsd, gcc, node, panda, php, qemu, linux, android},
xtick=data,
x tick label style={font=\scriptsize},
]
\addplot+[ybar,black!10,  fill=black!10]coordinates{(FFmpeg, 0.523395445) (freebsd, 0.660880792) (gcc,0.579552819) (node, 0.509130752) (panda, 0.703394546) (php, 0.731205303) (qemu, 0.679597114) (linux, 0.671470458) (android, 0.553839251)};
\addplot+[ybar,black!30,  fill=black!30]coordinates{(FFmpeg, 0.019047619) (freebsd, 0.002295223) (gcc,0.104180169) (node, 0.073776479) (panda, 0.007419774) (php, 0.013867085) (qemu, 0.017694297) (linux, 0.004200016) (android, 0.080694783)};
\addplot+[ybar,black!50,  fill=black!50]coordinates{(FFmpeg, 0.36563147) (freebsd, 0.288480849) (gcc,0.18713545) (node, 0.234477721) (panda, 0.19606752) (php, 0.180272109) (qemu, 0.192595617) (linux, 0.218955543) (android, 0.253236765)};
\addplot+[ybar,black!65,  fill=black!65]coordinates{(FFmpeg, 0.052173913) (freebsd, 0.030985511) (gcc,0.099481529) (node, 0.106647188) (panda, 0.05082545) (php, 0.038025467) (qemu, 0.065877229) (linux, 0.058313428) (android, 0.031790796)};
\addplot+[ybar,black!75,  fill=black!75]coordinates{(FFmpeg, 0.029813665) (freebsd, 0.01592311) (gcc, 0.029163966) (node, 0.073046019) (panda, 0.039695789) (php, 0.032618175) (qemu, 0.039063563) (linux, 0.046641685) (android, 0.074157159)};
\addplot+[ybar,black!100,  fill=black!100]coordinates{(FFmpeg, 0.009937888) (freebsd, 0.001434514) (gcc, 0.000486066) (node, 0.002921841) (panda, 0.002596921) (php, 0.004011861) (qemu, 0.005172179) (linux,0.00041887) (android, 0.006281246)};

\legend{P1, P2, P3, P4, P5, P6}
\end{axis}
\end{tikzpicture}



==> figure/groupRatio.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.45\textwidth]{figure/groupRatio.png}
\caption{The ratios of collaborative fixing commits grouped from security fixing and non-security fixing commits.}
\label{fig:groupRatio}
\vspace{-0.1in}
\end{figure}

==> figure/hero-dev-overlaps.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=0.5\textwidth]{figure/hero-dev-overlaps.png}
\caption{The overlap rates of ``top developers'' (i.e., contribute 80\% of a specific type of commits) between different types of commits.}
\label{fig:heor_overlap}
\end{figure}

==> figure/overlap_introcommits.tex <==
\begin{figure}[tb]
\centering
\includegraphics[width=0.45\textwidth]{figure/overlap_introcommits.png}
\caption{The overlap rate of non-security introducing commits and security introducing commits.}
\label{fig:overlap_introcommits}
\vspace{-0.1in}
\end{figure}

==> tab/heuristic.tex <==
\begin{table}[ht!]
\centering
\caption{Regular expression for identifying security-fixing commits.}
\label{tab:heuristic}
\begin{tabular}{|l|}
\hline
Regular Expression\\ \hline
\begin{tabular}[c]{@{}l@{}}(?i ) (denial .of.service |\textbackslash{}bXXE\textbackslash{}b|remote.code.execution|\textbackslash{}bopen.redirect |OSVDB|\textbackslash{}bvuln|\textbackslash{}bCVE\textbackslash{}b\\ |\textbackslash{}bXSS\textbackslash{}b|\textbackslash{}bReDoS\textbackslash{}b|\textbackslash{}bNVD\textbackslash{}b|malicious |x−frame−options |attack|cross.site |exploit |directory.\\ traversal |\textbackslash{}bRCE\textbackslash{}b|\textbackslash{}bdos\textbackslash{}b|\textbackslash{}bXSRF \textbackslash{}b|clickjack|session.fixation|hijack|advisory|insecure |security\\ |\textbackslash{}bcross−origin\textbackslash{}b|unauthori{[}z|s{]}ed|infinite.loop)\end{tabular} \\ \hline
\end{tabular}
\end{table}

==> tab/patternDiff.tex <==
\begin{table}[tb]
\centering
\caption{The difference of the percentages of interaction patterns between security activities and non-security activities.}
\label{tab:patternDiff}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{l|c|c|c|c|c|c}
\hline
Project & CoIntro & CoFix & IntroFix & SelfIntroFix & SelfIntro & SelfFix \\ \hline
FFmpeg  & -22.0   & 12.9  & -5.0     & -2.1         & 16.8      & -0.6    \\ 
freebsd & -25.7   & 11.2  & 1.4      & -0.5         & 13.7      & -0.1    \\ 
gcc     & -20.7   & 15.7  & 3.7      & -7.6         & 8.7       & 0.1     \\ 
node    & 8.1     & 18.9  & -13.7    & -9.1         & -3.9      & -0.2    \\ 
panda   & -30.9   & 3.4   & 16.0     & -1.1         & 12.7      & -0.1    \\ 
php     & -30.4   & 14.8  & 7.3      & 0.0          & 8.7       & -0.3    \\ 
qemu    & -32.5   & 17.9  & 9.2      & -2.2         & 8.0       & -0.4    \\ 
linux   & -35.0   & 15.0  & 11.1     & -2.3         & 11.2      & -0.1    \\ 
android & -26.3   & 12.8  & 2.6      & 2.5          & 8.9       & -0.5    \\ \hline
\end{tabular}
\vspace{-0.15in}
\end{table}

==> tab/projects-chro-firfox.tex <==
\begin{table*}[t!]
\centering
\caption{Experiment projects in this study. 
\textbf{Fix} is the number of commits that fixed security issues. 
\textbf{Intro} is the number of commits that 
introduced security issues.}
\label{tab:projects}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{Project} & \multirow{2}{*}{Language} & \multirow{2}{*}{LastCommitDate} & \multirow{2}{*}{\#Commit} & \multirow{2}{*}{\#Dev} & \multirow{2}{*}{\#CVE} & \multicolumn{3}{c|}{Security Vulners}  & \multicolumn{3}{c|}{General Bugs}      \\ \cline{7-12} 
           &             &     &        &          &        & \multicolumn{1}{c|}{Fix} & \multicolumn{1}{c|}{Intro} & \multicolumn{1}{c|}{Dev} & \multicolumn{1}{c|}{Fix} & \multicolumn{1}{c|}{Intro} & \multicolumn{1}{c|}{Dev} \\ \hline
Chromium   & C/C++       & 2018/11/05        & 729,992& 7,555    & 1,763  & 8,227      & 22,912       & 2,875 (38.05\%)    &     &&            \\ \hline
FireFox    & C/C++       & 2018/11/05        & 621,651& 6,981    & 1,771  & 3,850      & 8,517        & 1,298 (18.59\%)    &            &&            \\ \hline
Linux      & C/C++       & 2018/11/05        & 796,003& 19,362   & 2,207  & 10,316     & 17,126       & 3,686 (19.04\%)    &174,687     &313,804    &14,046       \\ \hline
PHP        & C/C++       & 2018/11/05        & 109,461& 911      & 588    & 979        & 1,292        & 165 (18.11\%)      &25,610      &48,296     &663          \\ \hline
FFmpeg     & C/C++       & 2018/11/05        & 92,349 & 1,713    & 308    & 810        & 1,007        & 199 (11.62\%)      &16,024		&26,592		&1,138        \\ \hline
Freebsd    & C/C++       & 2018/11/05        & 255,969& 766      & 341    & 2,640      & 4,086        & 386 (50.39\%)      &35,776      &66,490		&604          \\ \hline
Gcc        & C/C++       & 2018/11/05        & 165,475& 604      & 6      & 575        & 1,341        & 200 (33.11\%)      &15,836      &29,975     &506          \\ \hline
Panda      & C/C++       & 2018/11/05        & 52,580 & 1,220    & 24     & 557        & 1,072        & 230 (18.85\%)      &9,133       &17,125 	&838          \\ \hline
Qemu       & C/C++       & 2018/11/05        & 64,840 & 1,459    & 261    & 789        & 1,459        & 263 (18.03\%)      &12,139      &23,954     &1,023        \\ \hline
Android    & Java        & 2018/11/05        & 377,801& 2,938    & 1,763  & 2,439      & 2,521        & 496 (16.88\%)      &70,157		&128,893&2,132            \\ \hline
Nodejs     & JS          & 2018/11/05        & 24,401 & 2,640    & 48     & 252        & 402          & 105 (3.98\%)       &4,792       &10,571  	&1,302        \\ \hline
\end{tabular}

\end{table*}

==> tab/projects-old.tex <==
\begin{table*}[t!]
\centering
\caption{Experiment projects in this study. 
\textbf{Fix} is the number of commits that fixed security issues. 
\textbf{Intro} is the number of commits that 
introduced security issues.}
\label{tab:projects-old}
\begin{tabular}{|l|l|c|c|c|c|c|c|l|}
\hline
\multicolumn{1}{|c|}{\multirow{2}{*}{Project}} & \multicolumn{1}{c|}{\multirow{2}{*}{Language}} & \multirow{2}{*}{LastCommitDate} & \multirow{2}{*}{(CVE) Total Commits} & \multicolumn{2}{c|}{Security Commits} & \multirow{2}{*}{Percentage (\%)} & \multirow{2}{*}{Total Devs} & \multicolumn{1}{c|}{\multirow{2}{*}{Sec Devs}} \\ \cline{5-6}
\multicolumn{1}{|c|}{} & \multicolumn{1}{c|}{}  &  &  & Fix  & \multicolumn{1}{l|}{Intro}  &  & & \multicolumn{1}{c|}{}   \\ \hline

Chromium  & C/C++   & 2018/11/05       & (1,763) 729,992  & 8,227   & 22,912  & 4.27  & 7,555   & 2,875 (38.05\%) \\ \hline
FireFox   & C/C++, JS   & 2018/11/05       & (1,771) 621,651  & 3,850  &8,517 &  2.00   &  6,981   & 1,298 (18.59\%) \\ \hline
Linux     & C/C++   & 2018/11/05       & (2207) 796,003  & 10,316 &  17,126  &   3.45  & 19,362 & 3,686 (19.04\%) \\ \hline
PHP       & C/C++, PHP   & 2018/11/05 & (588) 109,461  & 979    & 1,292 &     2.07 &  911 & 165 (18.11\%) \\ \hline
FFmpeg    & C/C++   & 2018/11/05   & (308) 92,349   & 810   & 1,007 &  1.97 &  1,713  & 199 (11.62\%) \\ \hline
Freebsd   & C/C++   & 2018/11/05       & (341) 255,969  & 2,640   &   4,086 & 2.63 & 766 & 386 (50.39\%) \\ \hline
Gcc       & C/C++   & 2018/11/05      & (6) 165,475  & 575    &   1,341& 1.16  & 604  & 200 (33.11\%) \\ \hline
Panda     & C/C++   & 2018/11/05       &  (24) 52,580  &  557  & 1,072  &  3.10  & 1,220 & 230 (18.85\%) \\ \hline
Qemu      & C/C++   & 2018/11/05   & (261) 64,840  &  789  &   1,459   &   3.47  &  1,459 & 263 (18.03\%) \\ \hline
Andriod & Java & 2018/11/05   & (1,763) 377,801  & 2,439 & 2,251  & 1.24 &2,938 &496 (16.88\%) \\ \hline
Nodejs   & JavaScript  & 2018/11/05  &  (48) 24,401 &  252  & 402  &  2.68  & 2,640&  105 (3.98\%) \\ \hline
\end{tabular}
\end{table*}
